RSCC: A Large-Scale Remote Sensing Change Caption Dataset for Disaster Events

Remote sensing is critical for disaster monitoring, yet existing datasets lack temporal image pairs and detailed textual annotations. While single-snapshot imagery dominates current resources, it fails to capture dynamic disaster impacts over time. To address this gap, we introduce the Remote Sensing Change Caption (RSCC) dataset, a large-scale benchmark comprising 62,351 pre-/post-disaster image pairs (spanning earthquakes, floods, wildfires, and more) paired with rich, human-like change captions. By bridging the temporal and semantic divide in remote sensing data, RSCC enables robust training and evaluation of vision-language models for disaster-aware bi-temporal understanding. Our results highlight RSCC's ability to facilitate detailed disaster-related analysis, paving the way for more accurate, interpretable, and scalable vision-language applications in remote sensing. Code and dataset are available at https://github.com/Bili-Sakura/RSCC.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The abstract and introduction clearly state the contributions (RSCC dataset, rich annotations, experiments with MLLMs) and scope (disaster-awareness bi-temporal understanding). Claims align with experimental results and dataset statistics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:  \answerYes{}.
    \item[] Justification: Limitations are discussed in Section~\ref{sec:limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The paper focuses on dataset construction and empirical evaluation, with no theoretical claims or proofs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer:  \answerYes{}.
    \item[] Justification: The code and dataset are publicly available. The paper describes data sources, models, and evaluation metrics. Configurations for MLLMs' generation are detailed; full reproducibility relies on the GitHub repository.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The abstract states: "Code and dataset are available at https://github.com/Bili-Sakura/RSCC."
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer:  \answerYes{}.
    \item[] Justification: Inference configurations, data preprocessing and evaluation metrics are described in the main text.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer:  \answerNo{}.
    \item[] Justification:  We find only marginal performance differences using different random seeds to run experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer:  \answerYes{}.
    \item[] Justification: Details are shown in Section~\ref{sec:evaluation} and Appendeix~\ref{appendix}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer:  \answerYes{}.
    \item[] Justification: The dataset is sourced from MAXAR OpenData Program, which is publicly available. Ethical implications of disaster response applications are implicitly aligned with societal benefits.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}.
    \item[] Justification: We state broader impacts in Appendix~\ref{appendix}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}.
    \item[] Justification: The dataset is tailored for disaster analysis, with low inherent misuse risk. No safeguards are needed beyond standard licensing.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}.
    \item[] Justification: Existing datasets (xBD, EBD) are properly cited. Licenses for MAXAR OpenData and other sources are stated in Appendix~\ref{appendix}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}.
    \item[] Justification: The RSCC dataset and code are released on GitHub. Documentation (e.g., event lists, annotation protocols) is included in the paper and appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer:  \answerYes{}.
    \item[] Justification: Human preference study interface screenshots and guidelines are provided in Appendix~\ref{appendix}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer:  \answerNo{}.
    \item[] Justification: This work did not require IRB approval under [Country/Institution] guidelines, as it involved minimal-risk expert labeling of remote sensing data without sensitive or personal information collection. Participants were informed of the task requirements, and participation was voluntary. No identifiable data or compensation was involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{}.
    \item[] Justification: The paper uses QvQ-Max and other MLLMs for change caption generation, which is a core methodological component (Section~\ref{sec:pipeline}). This is explicitly declared in the methodology.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/methodology.tex <==
\section{Methodology}
OPERA~\citep{huangOPERAAlleviatingHallucination2024}, VCD~\citep{lengMitigatingObjectHallucinations2024}, PAI~\citep{liuPayingMoreAttention2024}

==> sections/prompt.tex <==
\begin{table*}[!ht]\centering
\begin{minipage}{0.85\textwidth}
%\vspace{0mm}    
\centering
\begin{tcolorbox} 
    \centering
   
     %\hspace{-4mm}
      \small
    \begin{tabular}{p{0.95\textwidth}}
   \textcolor[rgb]{0.8,0.3,0}{ {\bf SYSTEM:} } \\ 
    You are a helpful assistant. \\ \\
  \textcolor[rgb]{0.8,0.3,0}{ {\bf USER:} } \\ 
    Given a question and an answer in the VQA task, you are required to condense the answer into 1 to 5 words. You MUST FOLLOW THE FOLLOWING RULES: \\
    1. The condensed answer must be fewer than 5 tokens. \\
    2. The condensed answer must retain the core meaning of the original answer. \\
    3. Return only the condensed answer. DON'T RESPOND ANYTHING ELSE! \\ \\
    Here are some examples:\\
    <example 1>\\
    question: What is the current action and its justification? Answer in the form "action, justification".\\
    original answer: The car starts and moves right, because the vehicle in front is pulling away at the green traffic light and then it needs to go around the construction sign on the left of the road.\\
    condensed answer: Moves right.\\ \\
    <example 2> \\
    question: Is there a traffic light? If yes, what color is displayed? \\
    original answer: Yes, a temporary traffic light. It is showing green. \\
    condensed answer: Yes, green. \\
    \\
    <example 3> \\
    question: How many pedestrians are present in this image? \\
    original answer: There are no relevant pedestrians, but there is one on the left side-road and one on the right side of the road. \\
    condensed answer: No pedestrians. \\
    \\
    question: \{question\} \\
    original answer: \{answer\} \\
    condensed answer: 
    \\
    \end{tabular}
\end{tcolorbox}
%\vspace{-2mm}
\caption{Prompt template of answers simplification.}
\label{tab:simplify}
\end{minipage}
\end{table*}



\begin{table*}[!ht]\centering
\begin{minipage}{0.85\textwidth}
%\vspace{0mm}    
\centering
\begin{tcolorbox} 
    \centering
   
     %\hspace{-4mm}
      \small
    \begin{tabular}{p{0.95\textwidth}}
   \textcolor[rgb]{0.8,0.3,0}{ {\bf SYSTEM:} } \\ 
    You are a helpful assistant. \\ \\
  \textcolor[rgb]{0.8,0.3,0}{ {\bf USER:} } \\ 
   Given a question in the Automatic Driving QA task, you are required to rewrite the question in a different way. 
You MUST FOLLOW THE FOLLOWING RULES: \\
    1. The rephrased question should not have a high degree of overlap with the original wording. \\
    2. The rephrased question should be consistent with the core meaning of the original question. \\
    3. Return only the rephrased question. DON'T RESPOND ANYTHING ELSE! \\ \\
    
    Here are some examples: \\
    <example 1> \\
    original question: What is the current action and its justification? Answer in the form \"action, justification\". \\
    rephrased question: What is the action being performed at the moment, and what is the reasoning behind it? Please respond with "action, reasoning." \\ \\
    
    <example 2> \\
    original question: How many pedestrians are in the video? \\
    rephrased question: What is the number of pedestrians depicted in the video? \\ \\
    
    <example 3> \\
    original question: Is there a traffic light? If yes, what color is displayed? \\
    rephrased question: Does a traffic light exist, and if so, what is its current color? \\ \\
    
    original question: \{question\} \\
    rephrased question:

    \end{tabular}
\end{tcolorbox}
%\vspace{-2mm}
\caption{Prompt template of question rephrase.}
\label{tab:question}
\end{minipage}
\end{table*}



\begin{table*}[!ht]\centering
\begin{minipage}{0.85\textwidth}
%\vspace{0mm}    
\centering
\begin{tcolorbox} 
    \centering
     %\hspace{-4mm}
      \small
    \begin{tabular}{p{0.95\textwidth}}
   \textcolor[rgb]{0.8,0.3,0}{ {\bf SYSTEM:} } \\ 
    You are a helpful assistant. \\ \\
  \textcolor[rgb]{0.8,0.3,0}{ {\bf USER:} } \\ 
    Given a description about a road street view in Automatic Driving task, you are required to generate questions and provide corresponding answers from the description. \\
    You MUST FOLLOW THE FOLLOWING RULES: \\
    1. The questions must be related to driving from multiple perspectives, such as traffic object recognition, traffic condition analysis, and so on. \\
    2. The questions cannot be repeated. \\
    3. The corresponding answer must be condensed, such as fewer than 5 tokens. \\
    4. The content of the questions and answers must not include anything not covered in the description. \\
    5. Return only a series of Q\&A pairs in the form of a dictionary list. DON'T RESPOND ANYTHING ELSE! \\ \\
    Here are some examples: \\
    <example 1> \\
    description: In the traffic scene observed, there is one vehicle parked on the side of the road. Although it is partially obscured by darkness, it serves as an indication of a potentially active parking area where the ego car should remain vigilant for other vehicles that might enter or exit parking spots. Additionally, there is a traffic sign situated on the right that informs drivers of an upcoming pedestrian crossing. This suggests that the ego car should decrease its speed and be ready to yield to pedestrians who might be in the vicinity. \\
    Q\&A: [\{"question": "What should the ego car remain vigilant for?","answer": "Other vehicles entering/exiting"\},\{"question": "Where is the traffic sign located?","answer": "On the right"\},\{"question": "What does the traffic sign indicate?","answer": "Upcoming pedestrian crossing"\},\{"question": "What should the ego car do near the pedestrian crossing?","answer": "Decrease speed and yield"\}] \\

    <example 2> \\
    description: In the traffic image, there is a small black dog on the left side of the road ahead, appearing to cross from left to right. The dog's presence and potential for unpredictable movement pose a hazard, as animals can change direction suddenly, which could lead to an accident if the autonomous vehicle does not respond correctly. There are no vehicles, traffic signs, traffic lights, traffic cones, barriers, or other objects present in the image that affect driving behavior. \\
    Q\&A: [\{"question": "Are there any vehicles on the road?","answer": "No"\},\{"question": "Are there any traffic signs present?","answer": "No"\},\{"question": "Are there any barriers on the road?","answer": "No"\}]\\
    \\
    <example 3> \\
    description: The traffic scene contains a large cement mixer truck ahead on the road, taking up most of the driving lane. The truck is equipped with rear safety features like warning lights. This vehicle significantly impacts the driving behavior of the ego car, as its size and positioning affect the car's ability to safely overtake and necessitate maintaining a sufficient following distance. Additionally, there are construction barriers and debris on the side of the road to the right. These obstructions narrow the available road space, posing potential hazards that require the ego car to drive cautiously to avoid a collision. There are no vulnerable road users, traffic signs, traffic lights, traffic cones, or other objects present in this image that affect driving conditions. \\
    Q\&A: [\{"question": "What vehicle is ahead on the road?","answer": "Cement mixer truck"\},\{"question": "What safety features does the truck have?","answer": "Warning lights" \},\{"question": "How does the truck affect the ego car?","answer": "Impacts overtaking and following distance"\},\{"question": "What is on the right side of the road?","answer": "Construction barriers and debris"\},\{"question": "How do the obstructions on the right affect driving?","answer": "Narrow the road space"\},\{"question": "Are there any vulnerable road users present?","answer": "No" \},\{"question": "Are there any traffic signs or lights in the scene?","answer": "No"\}] \\
    \\
    description: \{description\} \\
    Q\&A: \\

    \end{tabular}
\end{tcolorbox}
%\vspace{-2mm}
\caption{Prompt template of general QA pairs self-generate.}
\label{tab:qa-general}
\end{minipage}
\end{table*}





\begin{table*}[!ht]\centering
\begin{minipage}{0.85\textwidth}
%\vspace{0mm}    
\centering
\begin{tcolorbox} 
    \centering
     %\hspace{-4mm}
      \small
    \begin{tabular}{p{0.95\textwidth}}
   \textcolor[rgb]{0.8,0.3,0}{ {\bf SYSTEM:} } \\ 
    You are a helpful assistant. \\ \\
  \textcolor[rgb]{0.8,0.3,0}{ {\bf USER:} } \\ 
    Given a driving suggestion about a road street view in Automatic Driving task, you are required to generate questions and provide corresponding answers from the description. \\
    You MUST FOLLOW THE FOLLOWING RULES: \\
    1. The questions must be related to driving from multiple perspectives, such as driving suggestion, traffic condition analysis, and so on. \\
    2. The questions cannot be repeated. \\
    3. The corresponding answer must be condensed, such as fewer than 5 tokens. \\
    4. The content of the questions and answers must not include anything not covered in the description. \\
    5. Return only a series of Q\&A pairs in the form of a dictionary list. DON'T RESPOND ANYTHING ELSE! \\
    \\
    Here are some examples: \\
    <example 1> \\
    suggestion: The ego car should reduce speed and prepare to stop if necessary, giving ample space for the dog to cross safely. Maintain vigilant observation of the dog's movements and be prepared for sudden changes in its direction. Furthermore, due to the narrowness and environment of the road, the ego car should drive cautiously, being alert for other potential obstacles or road users that may emerge from the side buildings or alleys. \\
    Q\&A: [\{"question": "What should the ego car do regarding speed?","answer": "Reduce speed"\},\{"question": "Why should the ego car drive cautiously?","answer": "Narrow road and potential obstacles"\},\{"question": "What other hazards should the driver be alert to?","answer": "Side buildings or alleys"\}] \\
    \\
    <example 2> \\
    suggestion: Given the proximity to the heavy vehicle ahead and the construction debris to the side, the ego car should maintain a safe following distance, prepare to slow down or stop if the mixer truck's behavior indicates impending stops or turns and refrain from attempting to overtake unless the opposite lane is visibly clear and safe to do so. The ego car should also be prepared for potential hazards from the construction area, such as entering construction vehicles or workers, and remain vigilant for any changes in road width or conditions. \\
    Q\&A: [\{"question": "What distance should the ego car maintain?","answer": "Safe following distance"\},\{"question": "What hazards should the driver be prepared for?","answer": "Construction vehicles or workers"\}] \\
    \\
    <example 3> \\
    suggestion: Given the wet road conditions, it is recommended that the ego car reduces its speed to ensure a safe stopping distance from the vehicle ahead. It should monitor the green traffic light for changes and be prepared to stop if it switches to yellow or red. The ego car should remain in the current lane, as the presence of vehicles in the left lane may hinder safe lane changing, and the road ahead seems to be leading to an exit which is partially blocked by barriers, making it inaccessible. Adherence to the road signage for navigation should be maintained, but no immediate action is required since there is no indication of an upcoming turn or exit that is accessible. Always be observant for any road users that might appear unexpectedly. \\
    Q\&A: [\{"question": "What should the ego car do due to wet road conditions?","answer": "Reduce speed"\},\{"question": "Which lane should the ego car stay in?","answer": "Current lane"\},\{"question": "Why should the ego car avoid changing lanes?","answer": "Left lane vehicles may hinder"\}] \\
    \\
    suggestion: \{suggestion\} \\
    Q\&A: \\
    \end{tabular}
\end{tcolorbox}
%\vspace{-2mm}
\caption{Prompt template of driving suggestion QA pairs self-generate.}
\label{tab:qa-driving}
\end{minipage}
\end{table*}
